Search for a Standard Model Higgs boson decaying to b quarks and produced in association with Z/W bosons with the CMS detector

A search for the standard model Higgs boson is performed in a data sample corresponding to an integrated luminosity of 1.1 fb$^{-1}$, recorded by the CMS detector in proton-proton collisions at the LHC with a 7 TeV center-of-mass energy. The following modes are studied: W($\mu \nu$)H, W(e$\nu$)H, Z($\mu \mu$)H, Z(ee)H and Z($\nu \nu$)H, with the Higgs decaying to bb pairs. 95% C.L. upper limits on the VH production cross section are derived for a Higgs mass between 110 and 135 GeV. The expected (observed) upper limit at 115 GeV is found to be 5.7 (8.3) times the standard model expectation.

==> HIG-11-012/trunk/HIG-11-012-BDT.tex <==
 The \BDT\ analysis is implemented in the TMVA framework~\cite{tmva}.
The training is done with simulated samples for signal and background
that pass a looser event selection relative to the \Mbb\ analyses. 
 Table~\ref{tab:BDTsel} 
summarizes the final selection of the \BDT\ analyses. Several input
variables were 
chosen by iterative optimization. These include the di-jet invariant
mass and momentum: \Mjj\ and \ptjj\ ,
the V transverse momentum \ptV\ , the CSV value for each of the two
jets, the azimuthal
angle between the V and the dijets, \dphiVH\ , and the pseudorapidity 
separation between the two jets, \dEtaJJ\ .
The \BDT\
 analysis was expected to improve the sensitivity with respect
to the \Mbb\ analysis by about 10\%
 in every channel.


\begin{table}[tbp]
\caption{Training selection and final signal region in each channel in 
the BDT analyses.  Entries marked ``--'' indicate that 
the variable is not used in the given channel.  For \ZnnH\ and \ZmmH\  the signal
window lower boundary was  optimized separately for each mass point
 (from 110 to 135): For \ZnnH\ the values are:  -0.160, -0.175,
 -0.215, -0.175, -0.185, -0.215, and the corresponding
\ZmmH\ values are: -0.198, -0.147, -0.147,
-0.198, -0.147, -0.198.}
\label{tab:BDTsel}
\begin{center}
\begin{tabular}{cccccc} \hline\hline
 Variable  & \WmnH    & \WenH	 & \ZmmH     & \ZeeH    & \ZnnH     \\ \hline
m$_{\ell\ell}$  &  --    & --	 & $75<$m$_{\ell\ell}<105$     & $75<$m$_{\ell\ell}<105$   & --    \\
$\pt(b_1)$ & $>30$    & $>30$	 & $>20$     & $>20$    & $>80$     \\
$\pt(b_2)$ & $>30$    & $>30$	 & $>20$     & $>20$    & $>20$     \\
\ptjj      & $>150$   & $>150$	 &  --       & --       & $>160$    \\
\ptV       & $>150$   & $>150$	 &  --       & --       & --	    \\
CSV1       & $>0.40$  & $>0.40$	 & $>0.24$   & $>0.24$  & $>0.50$   \\
CSV2       & $>0.40$  & $>0.40$  & $>0.24$   & $>0.24$  & $>0.50$   \\
\Naj       & --       & --  	 & $<2$      & $<2$     & --        \\
\Nal       & $=0$     & $=0$	 &  --       & --       & $=0$      \\
%\dphiVH    & --       & --       & $>2.4$    & $>2.4$   & --        \\
\dphiMJ    & --       & --       &  --       & --       & $>0.5$    \\
%pfMET      &    --    &	$>35$    &  --       & --       & --        \\
pfMETsig   &    --    &	$>2$       &  --       & --       & $>5$      \\
BDT        & $>0.050$  & $>0.040$  & variable  & $>0.160$  & variable  \\
\hline\hline
\end{tabular}
\end{center}
\end{table}




==> HIG-11-012/trunk/HIG-11-012-bck-ctrl.tex <==
Appropriate control regions that are orthogonal to the signal region are 
identified in data and used to adjust Monte Carlo estimates for 
the most important background processes: \Wj\ and \Zj\ (with
light and heavy-flavor jets), \ttbar\ and QCD
multijet and heavy-quark production.  Different control regions are
found for each of the different search channels by changing the event
selection in a way that enriches the content of each specific
background. For all cases, control regions with purity ranging 
from about 20\% to nearly 100\% have been successfully found. Discrepancies between the expected and 
observed yields in the data in these control regions are used to
obtain a scale factor by which the estimates from the simulation are
adjusted. The background from these sources in the signal region are then estimated from
the adjusted simulation samples, taking into account the associated
systematic uncertainty. The precise construction of all the control regions is involved and outside the 
scope of this summary note. The procedures applied include, for example: reversing the 
b-tagging requirements to enhance \Wj\ and \Zj\ with light-flavor jets; enforcing a tighter
b-tag requirement and requiring extra jets to enhance $t\bar t$ and requiring low ``boost'' in order
to enhance \Vbb\ over $t\bar t$ . Table~\ref{tab:MCSF} lists the control regions
and the corresponding purities and scale factors obtained.
Figure~\ref{fig:control_reg_ex_PAS} shows some examples of these
control regions for the \WlnH\ and the \ZllH\ analyses.


\begin{table}[tbp]
\caption{Purity and scale factors (Data/MC) derived from background
  enriched control regions, as described in the text. The scale
  factors for \WmnH\ and \WenH\ were averaged together, and the same
  was done for \ZmmH\ and \ZeeH.}
\label{tab:MCSF}
\begin{center}
\begin{tabular}{ccccccc}\hline\hline
 & \WmnH &    \WenH &     \WlnH       & \ZmmH &   \ZeeH &  \ZllH         \\ 
Control region  &  Purity  & Purity  & SF     &  Purity  & Purity  & SF \\ \hline
\Vudscg           & 80.2\% & 79.4\% & $0.84\pm 0.10$ & 92.8\% & 95.4\% & $0.88\pm 0.02$ \\ \hline
$t\bar t$          & 85.6\% & 85.8\% & $1.01\pm 0.11$ & 95.4\% & 97.5\% & $0.99\pm 0.05$ \\ \hline
V+$b\bar b$  & 20.1\% & 20.2\% & $1.40\pm 0.29$ & 83.7\% & 81.6\% & $1.16\pm 0.08 $   \\ \hline\hline
\end{tabular}
\end{center}
\end{table}


\begin{figure}[tbp]
  \begin{center}
    \includegraphics[width=0.46\textwidth]{figures/WenHWudscgNorm17.pdf}
    \includegraphics[width=0.46\textwidth,height=0.3\textheight]{figures/ZmmHZudscg2.pdf}
    \includegraphics[width=0.46\textwidth]{figures/WmnHTTbarNorm17.pdf}
    \includegraphics[width=0.46\textwidth]{figures/ZeeHTTbarPt.pdf}
    \includegraphics[width=0.46\textwidth]{figures/WenHWbbNorm17.pdf}
    \includegraphics[width=0.46\textwidth]{figures/ZmmHZbb2.pdf}
   \caption{
Distributions of dijet transverse momentum for events enhanced in production
of \Vudscg\ (top row), \ttbar\ (middle row), and \Vbb\ (bottom row).  Examples
are shown for events reconstructed as \WenH\ (top and bottom left), 
\WmnH\ (middle left), \ZmmH\ (top and bottom right), and \ZeeH\ (middle right).
Simulation is normalized to the data to facilitate the shape comparison.}
    \label{fig:control_reg_ex_PAS}
  \end{center}
\end{figure}


The \ZnnH\ channel is unique among the five modes analyzed, in that
it does not include charged leptons.  An important check is to 
compare the observed pfMET distribution with the predicted distribution
from simulation.  To accomplish this, muons are removed from the 
\ZmmJ\ data sample. 
In Fig.~\ref{fig:Znnctrl}, the resulting pfMET distribution is compared 
to \ZnnH\ simulated events.  Good overall agreement is 
found. 
Reasonably pure samples of \ttbar\ and \WJ\ events can be obtained by
requiring at least one additional isolated lepton in the event, and then
either requiring (for \ttbar) or vetoing (for \WJ) b-jets. 
Table~\ref{tab:MCSF_Zinv} 
lists the control regions and the corresponding purities and scale
factors obtained. Some of the corresponding distributions are shown in
Fig.~\ref{fig:Znnctrl}. 


The QCD background in the signal region is also estimated from data
using control regions of high and low values of two uncorrelated
variables with significant discriminating power towards QCD events.
One is the angle between the missing
energy vector and the closest jet in azimuth, \dphiMJ\, and the other
is the sum of the CSV values of the two b-tagged jets. The signal
region is at high values of both discriminants, while QCD populates
regions with low values of either. The method predicts a very small
contamination of $0.015\pm 0.008$
QCD background events, which we consider to be negligible.


\begin{table}[tbp]
\caption{$Z_{inv}$ Purity and scale factors (Data/MC) derived 
from background enriched control regions, as described in the text.}
\label{tab:MCSF_Zinv}
\begin{center}
\begin{tabular}{ccc}\hline\hline
Control region  &  Purity         & SF   \\ \hline\hline
\Zudscg           &    92.4\%        &   $0.97\pm 0.06$     \\ \hline
\Wudscg           &   94.1\%        &   $0.92\pm 0.05$     \\ \hline
\Zbb               &    44.4\%        &   $1.00\pm 0.30$     \\ \hline
$t\bar t$  &    89.9\%        &   $0.91\pm 0.09$     \\\hline
\end{tabular}
\end{center}
\end{table}


\begin{figure}[tbp]
  \begin{center}
%    \includegraphics[width=0.48\textwidth]{figures/ZnnHZudscg.pdf}
%    \includegraphics[width=0.48\textwidth]{figures/ZnnHTTbar.pdf}
%    \includegraphics[width=0.48\textwidth]{figures/ZnnHWjets.pdf}
    \includegraphics[width=0.48\textwidth]{figures/ZnnHZudscg_Aug19.pdf}
    \includegraphics[width=0.48\textwidth]{figures/ZnnHTTbar_Aug19.pdf}
    \includegraphics[width=0.48\textwidth]{figures/ZnnHWjets_Aug19.pdf}
   \caption{Examples of control regions for the \ZnnH\ analysis.
Dijet \pt distribution from a \ZmmJ\ data sample, with removed muons, 
compared to simulated \ZnnJ\ events (top left). Distribution of dijet invariant
 mass for the \ttbar\ (top right) and W+jets (bottom) control
 regions. The simulation has been normalized to the data.}
    \label{fig:Znnctrl}
  \end{center}
\end{figure}



==> HIG-11-012/trunk/HIG-11-012-conclusions.tex <==
This note reports the first cross section upper limits from the CMS experiment for standard model Higgs 
production in association with vector bosons and decaying to \bbbar\ pairs.  
A data sample corresponding to an integrated luminosity of $1.1$~fb$^{-1}$ has been analyzed in
these channels: \WmnH, \WenH, \ZmmH, \ZeeH, \ZnnH, and $95\%$ C.L.
upper limits were derived in a Higgs mass range from $110-135\GeV$ using the results from
the BDT analyses. At 115\GeV the expected (observed) upper limit is 5.7 (8.3)
times the standard model cross section.  These results can be directly compared to a
recent analysis from the ATLAS experiment~\cite{ATLASEPS2011}.



==> HIG-11-012/trunk/HIG-11-012-detector.tex <==
A detailed description of the CMS detector can be found
elsewhere~\cite{CMSDETECTOR}. The key components of the detector
include a silicon pixel and a silicon strip tracker, immersed in a 3.8~T
solenoidal magnetic field, which are used to measure the momenta of
charged particles. The tracker, which covers the pseudorapidity range
$|\eta| < 2.5$, is surrounded by a crystal electromagnetic calorimeter
(ECAL) and a brass-scintillator hadronic calorimeter (HCAL). The ECAL
and HCAL extend to a pseudorapidity range of $|\eta| < 3.0$. A quartz
fiber Cherenkov forward detector (HF) extends the calorimetric
coverage to $|\eta| < 5.0$. The outermost component of the CMS detector is the
muon system consisting of gas detectors placed in the iron return yoke
to measure the momentum of muons traversing through the detector.


==> HIG-11-012/trunk/HIG-11-012-event-rec.tex <==

The reconstructed interaction vertex with the largest value of
$\sum_i {\pt}_i^2$, amongst all reconstructed vertices, is selected as the primary event vertex (${\pt}_i$ is the transverse momentum of 
the $i$-th track in the vertex). The primary vertex is used as reference
for all other objects reconstructed in the event.

All relevant objects in the event are reconstructed offline with the
particle-flow algorithm. The extra PU interactions affect jet momentum reconstruction, \MET reconstruction, 
lepton isolation and b-tagging efficiency. To mitigate these effects
a track-based algorithm that filters all  charged hadrons that do not appear to
originate from the primary interaction is used. In addition a
calorimeter-based algorithm evaluates the energy density in the
calorimeter from interactions not related to the primary vertex and
subtracts it from reconstructed jets in the event.

Jets are defined as particle-flow objects clustered with the anti-\kt\ 
algorithm~\cite{antikt} using a size parameter of $0.5$.  Each jet is required to 
lie within $\left | \eta \right | < 2.5$, have at least two tracks associated to it, 
and have electromagnetic and hadronic energy fractions of at least $1\%$ of the total 
energy.  Standard jet-energy corrections are applied~\cite{jes}.

The \VEtmiss\ vector is calculated as the negative of the vectorial sum of transverse momenta of all particle-flow objects identified in the 
event, and the magnitude of this vector is referred to as pfMET.  This value divided by 
the square root of the scalar sum of \ET\ of all particle-flow objects is referred to as the 
``pfMET significance''. 


Electron reconstruction involves matching
particle-flow objetcs: energy clusters in the ECAL with tracks in the silicon
tracker~\cite{CMS-PAS-EGM-10-004}. Identification criteria based on the ECAL
shower shape, track-ECAL cluster matching and consistency with the
primary vertex are imposed.
%xxx anything on the vertex? on track quality?%
 Electron candidates that fall in the transition
region between ECAL barrel and endcap ($1.442 < |\eta| < 1.566$) are
rejected.  Additional requirements are imposed to remove electrons
produced by photon conversions. 
In this analysis electrons are considered in the pseudorapidity range $\left | \eta \right | < 2.5$,
excluding the gap region $1.44 < \left | \eta \right | < 1.57$. In
addition an isolation requirement is applied; the
sum of calorimeter energy and track momenta in a cone  of radius 0.4
around the electron is computed and electrons are rejected if this sum is
larger than 10\% of the electron momentum.
The electron reconstruction efficiency is close to~100\%.
 

Muons are reconstructed using two algorithms - one in which 
tracks in the silicon tracker are matched to hits in the muon
chamber and another in which a global track fit is performed seeded by
hits in the muon system~\cite{CMS-PAS-MUO-10-004}.  The muon
candidates used in the analysis are required to be reconstructed
successfully with both algorithms.  Further identification criteria
based on the number of hits in the tracker and the muon system, the
fit quality of the muon track and its consistency with the primary
vertex, are imposed on the muon candidates to reduce fakes.
The muon reconstruction efficiency is also close to~100\%.
%what about isolation?%

The CSV (``Combined Seconday Vertex'') b-tagging
algorithm~\cite{BTV-09-001,BTV-11-001} is used to identify jets that are likely to 
arise from the fragmentation and hadronization of b quarks.  This algorithm combines
in an optimal way the information about track impact parameters and secondary 
vertices within jets in a likelihood discriminant to provide maximal separation
of b-jets from jets originating from light quarks and gluons, and also
from charm quarks. The CSV output discriminant is continous and different 
optimal working points can be selected.

 All events from data and from the simulated samples are required to
pass the same trigger and event reconstruction algorithms. Scale
factors to account for the differences in the performance of these
algorithms between data and simulations are computed and used in
the analysis.


==> HIG-11-012/trunk/HIG-11-012-event-sel.tex <==

The main backgrounds to VH production include vector-boson plus heavy (W/Z+bb)
and light (W/Z+udscg) jets, \ttbar, single-top (ST), di-bosons (VV)
and QCD. These overwhelm the VH signal by several orders of magnitude. The signal event selection is therefore tight and it aims to
reconstruct kinematically the W/Z vector bosons and the Higgs decay
into two b-jets, while also reducing the background significantly. 
The event selection was optimized for significance, taking into
account available statistics (in the signal
and control regions) and the possible sculpting of the \Mbb\
distribution. We first describe the selection used to count events in the \Mbb\
analysis, and then the selection used to count events in the \BDT\
analysis. The final event selection for
each of the five channels considered was optimized separately. 



\subsection{Selection for the \Mbb\ Analysis}
Candidate \WtoLN\ decays are identified by requiring
the presence of a single, isolated, lepton and additional missing
transverse energy. Muons (electrons) are required to have a \pt\ above
20 (30)~GeV. Candidate \ZtoLL\ decays are reconstructed by combining 
isolated, opposite charge pairs of electrons and muons and requiring the dilepton invariant 
mass to satisfy $75<$m$_{\ell\ell}<105\GeV$.  For Z candidates the electron \pt\ is
lowered to 20~GeV.
The identification of \ZtoNN\ decays
requires pfMET~$>160\GeV$ (the high threshold dictated by the trigger).

The reconstruction of the \HBB\ decay is made by
requiring the presence of two central ($|\eta|<2.5$)
particle-flow jets, above a minimum \pt\ threshold and tagged by the
CSV algorithm. If more than two such jets are
found in the event, the pair with the highest sum of the CSV outputs
for the two jets is chosen (except for the WH analyses, in which
the $t\bar t$ background is larger, where the pair of jets with
highest total \pt\ is chosen). These combinations are found to yield
         higher efficiency and rejection of wrong combinations in signal
         events, as opposed to simply selecting the two highest \pt\ jets
         in the event. After b-tagging the fraction of \HBB\
         candidates that contain the two b-jets from the Higgs decay
         is near unity. For the tight CSV cut value ($>0.898$) used for b-tagging
         (see Table~\ref{tab:CCsel}) the efficiencies to tag
         b-quarks, c-quarks and light quarks were approximately 50\%,
         6\% and 0.15\%. The corresponding efficiencies for the looser
         CSV cut ($>0.5$) were approximately 72\%, 23\% and 3\%.

  
After b-tagging, the background from V+jets and di-bosons is reduced significantly and
becomes dominated by the sub-processes where the two jets originate from real b-quarks.
Events with additional jets (\Naj\ ) or additional leptons (\Nal\ ) are rejected to
further reduce backgrounds from \ttbar and WZ.

The topology of VH production is such that the W/Z
and the Higgs recoil away from each other with significant \pt. 
Cuts on the azimuthal opening angle between the vector 
boson and the reconstructed momenta of the Higgs candidate, \dphiVH,
on the \pt of the V-boson and on the b-tagged dijet pair
achieve significant rejection for most background processes and
improve the analysis reach.

For the  \ZtoNN\ channel, QCD backgrounds are further reduced
by a factor of $\sim 30$ when requiring that the pfMET does not originate from
mismeasured jets. A cut on the azimuthal angle between the pfMET and
the closest jet, $\dphiMJ>1.5$, is applied, together with the
requirement that pfMET significance be~$>5$.

Table~\ref{tab:CCsel} summarizes the selection criteria used in
each of the five channels. Table~\ref{tab:EffCC} summarizes the signal efficiency of the
selection criteria for the \Mbb\ analysis applied to each channel. 
All criteria are applied except for the trigger selection,
which is measured separately.  In addition, data/MC scale factors have
been determined for lepton reconstruction and identification efficiencies,
as well as the efficiency of tagging b-jets. 


\begin{table}[tbp]
\caption{Final selection applied to each channel in the \Mbb\
analyses, including the sliding windows on \Mjj\ for each mass point.  
Entries marked ``--'' indicate that there is no cut applied to the given 
variable in that channel.  The first two lines refer to the \pt\ threshold 
on the leading ($b_1$) and sub-leading ($b_2$) Higgs daughters, 
while CSV1\,(CSV2) are the max\,(min) b-tags for the two jets.}
\label{tab:CCsel}
\begin{center}
\begin{tabular}{cccc} \hline\hline
 Variable   & \WlnH        & \ZllH	  & \ZnnH	 \\ \hline
m$_{\ell\ell}$ &  --   & $75<$m$_{\ell\ell}<105$ & -- \\
$\pt(b_1)$  & $>30$        & $>20$	  & $>80$	 \\
$\pt(b_2)$  & $>30$        & $>20$	  & $>30$	 \\
\ptjj       & $>165$       & $>100$	  & $>160$	 \\
\ptV        & $>160$       & $>100$	  &  -- 	 \\
CSV1        & $>0.898$         &  $>0.898$	  &  $>0.898$	 \\
CSV2        & $>0.5$      & $>0.5$	  & $>0.5$	 \\
\dphiVH     & $>2.95$      & $>2.90$	  & $>2.90$	 \\
\Naj        & $=0$         & $<2$	  &  -- 	 \\
\Nal        & $=0$         &  --	  & $=0$	 \\
pfMET       & $>35$(\WenH)           &  --	  & $>160$	 \\
pfMETsig    & --           &  --	  & $>5$	 \\
\dphiMJ     & --           &  --	  & $>1.5$	 \\
$\Mjj(110)$ & $95$--$125$  & $90$--$120$  & $95$--$125$ \\
$\Mjj(115)$ & $100$--$130$ & $95$--$125$  & $100$--$130$ \\
$\Mjj(120)$ & $105$--$135$ & $100$--$130$ & $105$--$135$ \\
$\Mjj(125)$ & $110$--$140$ & $105$--$135$ & $110$--$140$ \\
$\Mjj(130)$ & $115$--$145$ & $110$--$140$ & $115$--$145$ \\
$\Mjj(135)$ & $120$--$150$ & $115$--$145$ & $120$--$150$ \\
\hline\hline
\end{tabular}
\end{center}
\end{table}



\begin{table}[tbp]
\caption{Signal efficiencies $(\%)$ for the \Mbb\ analysis selection in 
each channel as determined in the POWHEG signal Monte Carlo samples for 
$\MH=115\GeV$.  Each sample includes $220000$ events
produced. ``Pre-select'' includes all criteria described in the text
used to select the W/V/H bosons, other than those listed in this Table.
Entries marked with ``--'' indicate that the variable is not used
in the selection for that channel.  
The efficiency of each criterion is relative to the ones above. Uncertainties are statistical only.}
\label{tab:EffCC}
\begin{center}
\begin{tabular}{cccccc} \hline\hline
Pre-select & $13.40 \pm 0.07$ & $9.67  \pm 0.06$ & $12.88 \pm 0.07$ & $10.76 \pm 0.07$ & $20.02 \pm 0.09$ \\
\ptjj      & $11.70 \pm 0.19$ & $14.00 \pm 0.24$ & $28.50 \pm 0.27$ & $29.26 \pm 0.30$ & $23.51 \pm 0.20$ \\
\ptV       & $75.50 \pm 0.73$ & $78.29 \pm 0.76$ & $85.31 \pm 0.39$ & $85.65 \pm 0.42$ &     --           \\
CSV1       & $64.13 \pm 0.94$ & $62.58 \pm 1.00$ & $68.02 \pm 0.56$ & $68.46 \pm 0.60$ & $67.01 \pm 0.46$ \\
CSV2       & $55.75 \pm 1.22$ & $54.45 \pm 1.30$ & $59.17 \pm 0.72$ & $58.73 \pm 0.77$ & $63.51 \pm 0.58$ \\
\dphiVH    & $86.90 \pm 1.11$ & $90.44 \pm 1.04$ & $83.51 \pm 0.70$ & $83.57 \pm 0.76$ & $78.35 \pm 0.62$ \\
\Naj       & $74.78 \pm 1.53$ & $72.46 \pm 1.67$ & $92.57 \pm 0.55$ & $93.18 \pm 0.56$ &   --             \\
\Nal       & $100           $ & $100$            & --		    &	--	       & $99.88 \pm 0.06$ \\
pfMET      &	--	      & $88.34 \pm 1.43$ & --		    &	--	       & $76.31 \pm 0.72$ \\
pfMETsig   &	--	      & --		 & --		    &	--	       & $99.92 \pm 0.05$ \\
\dphiMJ    &	--	      & --		 & --		    &	--	       & $79.00 \pm 0.79$ \\
\Mjj       & $80.17 \pm 1.62$ & $81.38 \pm 1.71$ & $73.54 \pm 0.95$ & $73.20 \pm 1.03$ & $72.70 \pm 0.98$ \\\hline
Total Eff. & $ 0.22 \pm 0.01$ & $ 0.17 \pm 0.01$ & $0.72 \pm 0.02$  & $ 0.62 \pm 0.02$ & $ 0.69 \pm 0.02$ \\
\hline\hline
\end{tabular}
\end{center}
\end{table}


\subsection{BDT Selection}
\input{HIG-11-012-BDT.tex}


==> HIG-11-012/trunk/HIG-11-012-intro.tex <==
\label{sec:introduction}

The process by which the electroweak symmetry is broken in Nature remains elusive.
In the standard model (SM) the Higgs mechanism~\cite{ref:Higgs1,ref:Higgs2,ref:Higgs3} is
considered as the most likely explanation. The search for the Higgs boson is currently one of
the most important undertakings of experimental particle physics.

Measurements of the W and top-quark masses at LEP
and the Tevatron, combined with precision measurements of 
electroweak parameters at the Z pole, provide an indirect constraint 
on the Higgs mass of $\mH < 158\GeV$ at $95\%$ confidence level 
(C.L.)~\cite{LEPewkfits}.  Previous direct searches at the LEP 
experiments set a lower bound of $\mH > 114.4\GeV$ at 
$95\%$ C.L.~\cite{LEPHIGGS}, while direct searches at the Tevatron 
currently exclude the region $156$--$177\GeV$~\cite{ref:TEVsummer2011}, 
also at $95\%$ C.L.

Preliminary search results from 
CMS~\cite{HIG-11-003,HIG-11-004,HIG-11-005,HIG-11-006,HIG-11-009,HIG-11-010} 
and ATLAS~\cite{ATLAScomboEPS2011} are excluding even higher masses, and are starting to broaden 
the exclusion region near $165\GeV$. The most likely mass for the SM
Higgs is therefore at ``low mass'' near the LEP limit, where the Higgs decays
predominantly into $b\bar{b}$ pairs. 

At the LHC the main Higgs production mechanism is direct production through gluon fusion,
with a cross section of $\sim 17\cdot 10^3$~fb for a Higgs mass $\mH
= 120$~GeV~\cite{Dawson:1990zj,Spira:1995rr,Harlander:2002wh,Anastasiou:2002yz,Ravindran:2003um,Catani:2003zt,Actis:2008ug,Ciccolini:2007jr,Ciccolini:2007ec,Figy:2003nv,Arnold:2008rz,Bolzoni:2010xr,Anastasiou:2008tj,deFlorian:2009hc,hdecay2,LHCXSWG}.
However, in this production mode, the detection of the $H\to b\bar b$ decay
is rendered nearly impossible due to overwhelming QCD di-jet production.
The same holds true for the next most copious production mode, through
vector-boson fusion, with a cross section of $\sim1,300$~fb. Processes in which the Higgs is produced in association with a vector boson have cross sections
of $\sim660$ and $\sim360$~fb for $WH$ and $ZH$ respectively. Until
now these $VH$ processes, with $H\to b\bar b$, have not been considered as promising, in terms of
sensitivity, as the relatively more clean, but heavily suppressed,
final states: $H\to\gamma\gamma$ and $H\to\tau\tau$. Even if this is
the case, it is paramount to search for the Higgs in
these modes given that the observation of the $H\to b\bar b$ decay is
key to determine the nature of this particle, if and when discovered.

In this note a summary of a search for the standard model Higgs
boson in the $pp\to VH$ production mode is presented. The analysis
is performed in a data sample corresponding to an integrated luminosity of
 $1.1$~fb$^{-1}$, collected by the CMS experiment at a
7~TeV center-of-mass energy. The following final states are included:
$W(\mu\nu)H$, $W(e\nu)H$, $Z(\mu\mu)H$, $Z(ee)H$ and $Z(\nu\nu)H$
 --all with the Higgs decaying to $b\bar{b}$ pairs. 

Backgrounds arise from production of W and Z bosons associated with
jets (all flavors), singly and pair-produced top quarks, and di-bosons.  
Simulated samples of all backgrounds are used to provide
guidance in the analysis optimization, and an initial evaluation 
of their contributions in the search region.
For the main backgrounds, high-purity control regions are used to
estimate their contribution in the signal region.


An optimization of the event selection, that depends on the Higgs mass, is performed, and 95\%
C.L. upper limits on the  $pp\to VH$ production cross section are
obtained for Higgs masses between
110-135 GeV. These limits are based on the observed event count and background estimate in signal 
regions defined in either the invariant mass distribution of $H\to
b\bar b$ candidates (``\Mbb\, or cut-and-count analysis''), or in the output
discriminant of a boosted decision tree algorithm (``\BDT\ analysis''). The latter enhances
the statistical power of the analysis by making full use of correlations between discriminating 
variables in signal and background events.







==> HIG-11-012/trunk/HIG-11-012-results.tex <==
The final predicted number of events in the signal regions of the
BDT and \Mbb\ analyses are determined with a mix of data-driven
estimates based on the control regions described in Sec.~\ref{sec:bck-ctrl}, 
and expectations from simulation.  This section summarizes all of the
final signal and background estimates in both sets of analyses, including
the systematic uncertainties summarized in the previous section, and the
expected and observed upper limits using 1.1~fb$^{-1}$ of integrated luminosity.
The analyses were performed blind, in the sense that the analysis selection
was decided and frozen before the signal region in each channel was investigated.

\subsection{Signal and background estimates}

Tables~\ref{tab:WmnHCCyields}-\ref{tab:ZnnHCCyields} summarize the expected 
signal and background yields, and the observed number of events, in the signal 
region for each channel for the \Mbb\ analyses. Tables~\ref{tab:WmnHBDTYields}-\ref{tab:ZnnHBDTYields} summarize the expected 
signal and background yields, and the observed number of events, in the signal 
region for the \BDT\ analyses.  The BDT is retrained separately at each mass
point.  Single-top backgrounds are labeled ``ST'' in all tables.  The QCD 
background contribution was found to be negligible in all channels and is 
not listed.

The final \Mbb\ distributions and the final BDT distributions are shown in
Fig.~\ref{fig:MassCC} and in  Fig.~\ref{fig:BDTdata}, respectively.
The data is overlaid with the predicted background normalization. 

\begin{table}[htbp]
\caption{Predicted backgrounds including the statistical uncertainty and the
systematic uncertainty from the control region and b-tag scale factors, signal 
yields with total uncertainty, and the observed number of events for each mass 
point in the \WmnH\ \Mjj\ analysis.}
\label{tab:WmnHCCyields}
\begin{center}
\scalebox{0.8}{
\begin{tabular}{ccccccc} \hline\hline
Process     & $110\GeV$        & $115\GeV$        & $120\GeV$        & $125\GeV$        & $130\GeV$   & $135\GeV$        \\\hline
\Wudscg     & $0.105\pm 0.050$ & $0.081\pm 0.038$ & $0.068\pm 0.032$ & $0.045\pm 0.021$ & $0.061\pm 0.029$ & $0.096\pm 0.045$ \\
\Wbb        & $0.876\pm 0.233$ & $0.829\pm 0.221$ & $0.796\pm 0.212$ & $0.703\pm 0.187$ & $0.572\pm 0.152$ & $0.516\pm 0.137$ \\
Z+jets      & $0.178\pm 0.127$ & $0.184\pm 0.131$ & $0.006\pm 0.004$ & $0.252\pm 0.180$ & $0.252\pm 0.180$ & $0.252\pm 0.180$ \\
\ttbar      & $1.17 \pm 0.303$ & $1.109\pm 0.287$ & $1.207\pm 0.313$ & $1.232\pm 0.319$ & $1.107\pm 0.287$ & $1.209\pm 0.313$ \\
ST          & $0.254\pm 0.111$ & $0.24 \pm 0.105$ & $0.25 \pm 0.109$ & $0.271\pm 0.118$ & $0.285\pm 0.124$ & $0.223\pm 0.097$ \\
VV          & $0.244\pm 0.102$ & $0.153\pm 0.064$ & $0.039\pm 0.016$ & $0.021\pm 0.009$ & $0.017\pm 0.007$ & $0.009\pm 0.004$ \\\hline
\Bexp       & $2.827\pm 0.482$ & $2.596\pm 0.449$ & $2.366\pm 0.434$ & $2.524\pm 0.461$ & $2.294\pm 0.421$ & $2.305\pm 0.428$ \\\hline
WH          & $0.378\pm 0.106$ & $0.354\pm 0.099$ & $0.296\pm 0.083$ & $0.236\pm 0.066$ & $0.187\pm 0.052$ & $0.143\pm 0.040$ \\\hline
ZH          & $0.006\pm 0.002$ & $0.006\pm 0.002$ & $0.006\pm 0.002$ & $0.005\pm 0.001$ & $0.003\pm 0.001$ & $0.002\pm 0.001$ \\\hline
\Nobs       & $2$	       & $4$   	          & $4$              &      $4$         & $3$              & $3$              \\
\hline\hline
\end{tabular}
}
\end{center}
\end{table}

\begin{table}[htbp]
\caption{Predicted backgrounds including the statistical uncertainty and the
systematic uncertainty from the control region and b-tag scale factors, signal 
yields with total uncertainty, and the observed number of events for each mass 
point in the \WenH\ \Mjj\ analysis.}
\label{tab:WenHCCyields}
\begin{center}
\scalebox{0.8}{
\begin{tabular}{ccccccc} \hline\hline
Process     & $110\GeV$        & $115\GeV$        & $120\GeV$        & $125\GeV$        & $130\GeV$        & $135\GeV$        \\\hline
\Wudscg     & $0.036\pm 0.015$ & $0.01 \pm 0.004$ & $0.011\pm 0.004$ & $0.013\pm 0.005$ & $0.012\pm 0.005$ & $0.027\pm 0.011$ \\
\Wbb        & $0.442\pm 0.120$ & $0.344\pm 0.093$ & $0.375\pm 0.102$ & $0.370\pm 0.100$ & $0.32 \pm 0.087$ & $0.265\pm 0.072$ \\
Z+jets      & $0.204\pm 0.146$ & $0.204\pm 0.146$ & $0$              & $0$	        & $0$	           & $0$              \\
\ttbar      & $0.767\pm 0.193$ & $0.543\pm 0.136$ & $0.543\pm 0.136$ & $0.503\pm 0.126$ & $0.568\pm 0.143$ & $0.403\pm 0.101$ \\
ST          & $0.076\pm 0.030$ & $0.122\pm 0.049$ & $0.181\pm 0.072$ & $0.283\pm 0.113$ & $0.32 \pm 0.128$ & $0.385\pm 0.154$ \\
VV          & $0.134\pm 0.053$ & $0.065\pm 0.026$ & $0.045\pm 0.018$ & $0.042\pm 0.017$ & $0.033\pm 0.013$ & $0.029\pm 0.012$ \\\hline
\Bexp       & $1.66 \pm 0.299$ & $1.288\pm 0.242$ & $1.155\pm 0.206$ & $1.211\pm 0.217$ & $1.253\pm 0.228$ & $1.109\pm 0.209$ \\\hline
WH          & $0.263\pm 0.074$ & $0.296\pm 0.083$ & $0.203\pm 0.057$ & $0.201\pm 0.056$ & $0.142\pm 0.040$ & $0.123\pm 0.034$ \\\hline
ZH          & $0.004\pm 0.001$ & $0.002\pm 0.001$ & $0.003\pm 0.001$ & $0.002\pm 0.001$ & $0.002\pm 0.001$ & $0.001\pm 0.001$ \\\hline
\Nobs       & $4$	       & $4$              & $1$              & $1$              & $0$              & $0$	    \\
\hline\hline
\end{tabular}
}
\end{center}
\end{table}

\begin{table}[htbp]
\caption{Predicted backgrounds including the statistical uncertainty and the
systematic uncertainty from the control region and b-tag scale factors, signal 
yields with total uncertainty, and the observed number of events for each mass 
point in the \ZmmH\ \Mjj\ analysis.}
\label{tab:ZmmHCCyields}
\begin{center}
\scalebox{0.8}{
\begin{tabular}{ccccccc} \hline\hline
Process      & $110\GeV$        & $115\GeV$        & $120\GeV$        & $125\GeV$	 & $130\GeV$        & $135\GeV$        \\\hline
\Zudscg      & $0.110\pm 0.064$ & $0.110\pm 0.065$ & $0.110\pm 0.065$ & $0.110\pm 0.065$ & $0.150\pm 0.069$ & $0.110\pm 0.065$ \\
\Zbb         & $1.930\pm 0.337$ & $2.050\pm 0.396$ & $1.650\pm 0.373$ & $1.740\pm 0.378$ & $1.660\pm 0.375$ & $1.600\pm 0.361$ \\
\ttbar\ + ST  & $0.030\pm 0.031$ & $0.090\pm 0.036$ & $0.140\pm 0.044$ & $0.140\pm 0.044$ & $0.190\pm 0.053$ & $0.190\pm 0.127$ \\	
VV           & $0.260\pm 0.100$ & $0.160\pm 0.064$ & $0.070\pm 0.033$ & $0.030\pm 0.023$ & $0.020\pm 0.021$ & $0.010\pm 0.011$ \\\hline
\Bexp        & $2.330\pm 0.363$ & $2.410\pm 0.358$ & $1.970\pm 0.348$ & $2.020\pm 0.348$ & $2.020\pm 0.351$ & $1.910\pm 0.356$ \\\hline
$S$          & $0.218\pm 0.057$ & $0.195\pm 0.051$ & $0.152\pm 0.040$ & $0.128\pm 0.033$ & $0.102\pm 0.027$ & $0.077\pm 0.020$ \\\hline
\Nobs        & $3$              & $3$	           & $3$	      & $3$		 & $2$  	    & $3$	\\
\hline\hline
\end{tabular}
}
\end{center}
\end{table}


\begin{table}[htbp]
\caption{Predicted backgrounds including the statistical uncertainty and the
systematic uncertainty from the control region and b-tag scale factors, signal 
yields with total uncertainty, and the observed number of events for each mass 
point in the \ZeeH\ \Mjj\ analysis.}
\label{tab:ZeeHCCyields}
\begin{center}
\scalebox{0.8}{
\begin{tabular}{ccccccc} \hline\hline
Process      & $110\GeV$        & $115\GeV$        & $120\GeV$        & $125\GeV$        & $130\GeV$        & $135\GeV$        \\\hline
\Zudscg      & $0.013\pm 0.006$ & $0.006\pm 0.003$ & $0.004\pm 0.003$ & $0.007\pm 0.004$ & $0.024\pm 0.012$ & $0.028\pm 0.013$ \\
\Zbb         & $1.327\pm 0.173$ & $1.545\pm 0.254$ & $1.300\pm 0.214$ & $1.472\pm 0.242$ & $1.581\pm 0.250$ & $1.372\pm 0.217$ \\
\ttbar       & $0.105\pm 0.052$ & $0.133\pm 0.073$ & $0.090\pm 0.050$ & $0.090\pm 0.050$ & $0.070\pm 0.044$ & $0.070\pm 0.044$ \\
ST           & $0.009\pm 0.007$ & $0.009\pm 0.007$ & $0.028\pm 0.022$ & $0.019\pm 0.020$ & $0.019\pm 0.020$ & $0.019\pm 0.020$ \\
VV           & $0.236\pm 0.091$ & $0.189\pm 0.074$ & $0.104\pm 0.041$ & $0.066\pm 0.027$ & $0.037\pm 0.016$ & $0.024\pm 0.011$ \\\hline
\Bexp        & $1.690\pm 0.209$ & $1.883\pm 0.232$ & $1.526\pm 0.186$ & $1.655\pm 0.203$ & $1.731\pm 0.201$ & $1.513\pm 0.177$ \\\hline
$S$          & $0.211\pm 0.055$ & $0.193\pm 0.050$ & $0.148\pm 0.038$ & $0.136\pm 0.035$ & $0.102\pm 0.027$ & $0.081\pm 0.021$ \\\hline
\Nobs        & $1$              & $2$              & $2$              & $2$              & $3$              & $4$	       \\
\hline\hline
\end{tabular}
}
\end{center}
\end{table}

\begin{table}[htbp]
\caption{Predicted backgrounds including the statistical uncertainty and the
systematic uncertainty from the control region and b-tag scale factors, signal 
yields with total uncertainty, and the observed number of events for each mass 
point in the \ZnnH\ \Mjj\ analysis.}
\label{tab:ZnnHCCyields}
\begin{center}
\scalebox{0.8}{
\begin{tabular}{ccccccc} \hline\hline
Process       & $110\GeV$        & $115\GeV$        & $120\GeV$        & $125\GeV$        & $130\GeV$        & $135\GeV$        \\\hline
\Wudscg       & $0.024\pm 0.007$ & $0.023\pm 0.007$ & $0.022\pm 0.007$ & $0.019\pm 0.006$ & $0.014\pm 0.004$ & $0.012\pm 0.004$ \\
\Wbb + \ttbar & $2.030\pm 0.609$ & $1.780\pm 0.534$ & $2.050\pm 0.615$ & $2.360\pm 0.708$ & $2.420\pm 0.726$ & $2.110\pm 0.633$ \\
\Zudscg       & $0.180\pm 0.039$ & $0.180\pm 0.039$ & $0.140\pm 0.030$ & $0.130\pm 0.028$ & $0.120\pm 0.026$ & $0.130\pm 0.028$ \\
\Zbb          & $1.970\pm 0.603$ & $1.890\pm 0.578$ & $1.790\pm 0.548$ & $1.710\pm 0.523$ & $1.780\pm 0.545$ & $1.810\pm 0.554$ \\
ST            & $0.460\pm 0.174$ & $0.460\pm 0.174$ & $0.410\pm 0.155$ & $0.410\pm 0.155$ & $0.460\pm 0.174$ & $0.400\pm 0.152$ \\
VV            & $0.770\pm 0.292$ & $0.460\pm 0.174$ & $0.410\pm 0.155$ & $0.110\pm 0.042$ & $0.080\pm 0.030$ & $0.070\pm 0.027$ \\\hline
\Bexp         & $5.434\pm 1.069$ & $4.793\pm 0.938$ & $4.822\pm 0.958$ & $4.739\pm 0.969$ & $4.874\pm 0.998$ & $4.532\pm 0.918$ \\\hline
$S$           & $0.669\pm 0.174$ & $0.593\pm 0.154$ & $0.417\pm 0.108$ & $0.442\pm 0.115$ & $0.326\pm 0.085$ & $0.245\pm 0.064$ \\\hline
\Nobs         & $6$              & $5$	     	    & $5$   	     & $5$   	          & $6$              & $5$              \\
\hline\hline
\end{tabular}
}
\end{center}
\end{table}




\begin{table}[htbp]
\caption{Predicted backgrounds including the statistical uncertainty and the
systematic uncertainty from the control region and b-tag scale factors, signal 
yields with total uncertainty, and the observed number of events for each mass 
point in the \WmnH\ BDT analysis.}
\label{tab:WmnHBDTYields}
\begin{center}
\scalebox{0.8}{
\begin{tabular}{ccccccc} \hline\hline
Process     & $110\GeV$   & $115\GeV$        & $120\GeV$        & $125\GeV$        & $130\GeV$        & $135\GeV$               \\\hline
\Wudscg     & $0.661\pm 0.191$ & $0.667\pm 0.192$ & $0.546\pm 0.157$ & $0.628\pm 0.181$ & $0.697 \pm 0.201$ & $0.446 \pm 0.129$ \\
\Wbb        & $2.460\pm 0.644$ & $2.035\pm 0.533$ & $2.083\pm 0.545$ & $2.698\pm 0.706$ & $2.086 \pm 0.546$ & $2.450 \pm 0.641$ \\
Z+jets      & $0$              & $0.006\pm 0.006$ & $0.190\pm 0.190$ & $0.367\pm 0.368$ & $0.245 \pm 0.246$ & $0.190 \pm 0.190$ \\
\ttbar      & $1.667\pm 0.432$ & $1.173\pm 0.304$ & $1.362\pm 0.353$ & $2.239\pm 0.580$ & $2.262 \pm 0.586$ & $2.196 \pm 0.569$ \\
ST          & $0.608\pm 0.243$ & $0.653\pm 0.261$ & $0.673\pm 0.269$ & $0.956\pm 0.382$ & $1.007 \pm 0.402$ & $1.055 \pm 0.421$ \\
VV          & $0.496\pm 0.195$ & $0.355\pm 0.140$ & $0.345\pm 0.136$ & $0.283\pm 0.111$ & $0.216 \pm 0.085$ & $0.159 \pm 0.063$ \\\hline
\Bexp       & $5.892\pm 0.980$ & $4.889\pm 0.806$ & $5.199\pm 0.857$ & $7.171\pm 1.206$ & $6.513 \pm 1.074$ & $6.496 \pm 1.100$ \\\hline
WH          & $0.619\pm 0.173$ & $0.587\pm 0.164$ & $0.499\pm 0.140$ & $0.416\pm 0.116$ & $0.383 \pm 0.107$ & $0.281 \pm 0.079$ \\\hline
ZH          & $0.015\pm 0.004$ & $0.011\pm 0.003$ & $0.012\pm 0.003$ & $0.011\pm 0.003$ & $0.007 \pm 0.002$ & $0.006 \pm 0.002$ \\\hline
\Nobs       & $9$              & $7$              & $6$              & $5$              & $11$              & $11$	      \\
\hline\hline
\end{tabular}
}
\end{center}
\end{table}

\begin{table}[htbp]
\caption{Predicted backgrounds including the statistical uncertainty and the
systematic uncertainty from the control region and b-tag scale factors, signal 
yields with total uncertainty, and the observed number of events for each mass 
point in the \WenH\ BDT analysis.}
\label{tab:WenHBDTYields}
\begin{center}
\scalebox{0.8}{
\begin{tabular}{ccccccc} \hline\hline
Process     & $110\GeV$        & $115\GeV$        & $120\GeV$        & $125\GeV$        & $130\GeV$        & $135\GeV$        \\\hline
\Wudscg     & $0.148\pm 0.060$ & $0.155\pm 0.063$ & $0.241\pm 0.097$ & $0.300\pm 0.121$ & $0.342\pm 0.138$ & $0.220\pm 0.089$ \\
\Wbb        & $1.112\pm 0.302$ & $1.378\pm 0.374$ & $1.015\pm 0.276$ & $1.390\pm 0.377$ & $0.962\pm 0.261$ & $1.063\pm 0.289$ \\
Z+jets      & $0$              & $0.198\pm 0.141$ & $0.198\pm 0.141$ & $0.238\pm 0.170$ & $0.198\pm 0.141$ & $0.198\pm 0.141$ \\
\ttbar      & $0.790\pm 0.198$ & $1.254\pm 0.315$ & $2.037\pm 0.511$ & $2.008\pm 0.504$ & $1.996\pm 0.501$ & $2.533\pm 0.636$ \\
ST          & $0.381\pm 0.152$ & $0.653\pm 0.261$ & $0.658\pm 0.263$ & $0.920\pm 0.367$ & $1.081\pm 0.431$ & $1.268\pm 0.506$ \\
VV          & $0.343\pm 0.137$ & $0.292\pm 0.117$ & $0.232\pm 0.093$ & $0.201\pm 0.080$ & $0.151\pm 0.060$ & $0.138\pm 0.055$ \\\hline
\Bexp       & $2.774\pm 0.476$ & $3.930\pm 0.658$ & $4.381\pm 0.742$ & $5.057\pm 0.849$ & $4.730\pm 0.811$ & $5.420\pm 0.954$ \\\hline
WH          & $0.441\pm 0.123$ & $0.477\pm 0.134$ & $0.393\pm 0.110$ & $0.344\pm 0.096$ & $0.274\pm 0.077$ & $0.233\pm 0.065$ \\\hline
ZH          & $0.005\pm 0.001$ & $0.004\pm 0.001$ & $0.007\pm 0.002$ & $0.006\pm 0.002$ & $0.004\pm 0.001$ & $0.004\pm 0.001$ \\\hline
\Nobs       & $6$	       & $9$  	     	  & $7$  	     & $9$      	& $5$              & $5$  	    \\
\hline\hline
\end{tabular}
}
\end{center}
\end{table}

\begin{table}[htbp]
\caption{Predicted backgrounds including the statistical uncertainty and the
systematic uncertainty from the control region and b-tag scale factors, signal 
yields with total uncertainty, and the observed number of events for each mass 
point in the \ZmmH\ BDT analysis.}
\label{tab:ZmmHBDTYields}
\begin{center}
\scalebox{0.8}{
\begin{tabular}{ccccccc} \hline\hline
Process      & $110\GeV$        & $115\GeV$        & $120\GeV$        & $125\GeV$	 & $130\GeV$        & $135\GeV$         \\\hline
\Zudscg      & $2.023\pm 0.575$ & $1.225\pm 0.490$ & $1.002\pm 0.426$ & $0.696\pm 0.395$ & $0.585\pm 0.386$ & $0.341\pm 0.225$  \\
\Zbb         & $4.470\pm 0.621$ & $2.858\pm 0.645$ & $3.435\pm 0.776$ & $2.772\pm 0.746$ & $2.386\pm 0.707$ & $4.245\pm 0.854$  \\
\ttbar       & $0.409\pm 0.225$ & $0.296\pm 0.218$ & $0.460\pm 0.278$ & $0.601\pm 0.293$ & $0.684\pm 0.304$ & $0.873\pm 0.410$  \\
ST           & $0.060\pm 0.064$ & $0.060\pm 0.064$ & $0.060\pm 0.064$ & $0$ & $0.060\pm 0.064$ & $0.060\pm 0.064$  \\
VV           & $0.636\pm 0.243$ & $0.334\pm 0.130$ & $0.507\pm 0.197$ & $0.344\pm 0.141$ & $0.089\pm 0.052$ & $0.161\pm 0.065$  \\\hline
\Bexp        & $7.598\pm 1.018$ & $4.773\pm 0.841$ & $5.464\pm 0.938$ & $4.413\pm 0.896$ & $3.804\pm 0.855$ & $5.680\pm 0.902$  \\\hline
$S$          & $0.440\pm 0.114$ & $0.328\pm 0.085$ & $0.295\pm 0.077$ & $0.244\pm 0.063$ & $0.164\pm 0.043$ & $0.148\pm 0.038$  \\\hline
\Nobs        & $9$              & $4$   	   & $7$              & $4$              & $4$   	    & $7$               \\
\hline\hline
\end{tabular}
}
\end{center}
\end{table}


\begin{table}[htbp]
\caption{Predicted backgrounds including the statistical uncertainty and the
systematic uncertainty from the control region and b-tag scale factors, signal 
yields with total uncertainty, and the observed number of events for each mass 
point in the \ZeeH\ BDT analysis.}
\label{tab:ZeeHBDTYields}
\begin{center}
\scalebox{0.8}{
\begin{tabular}{ccccccc} \hline\hline
Process      & $110\GeV$        & $115\GeV$        & $120\GeV$        & $125\GeV$        & $130\GeV$        & $135\GeV$         \\\hline
\Zudscg      & $0.459\pm 0.174$ & $0.077\pm 0.036$ & $0.120\pm 0.056$ & $0.140\pm 0.058$ & $0.290\pm 0.116$ & $0.310\pm 0.116$  \\
\Zbb         & $0.699\pm 0.129$ & $0.904\pm 0.189$ & $1.117\pm 0.216$ & $1.040\pm 0.193$ & $1.441\pm 0.268$ & $1.535\pm 0.274$  \\
\ttbar       & $0.223\pm 0.121$ & $0.179\pm 0.133$ & $0.455\pm 0.284$ & $0$ & $0.286\pm 0.213$ & $0.170\pm 0.127$  \\
ST           & $0.002\pm 0.001$ & $0$ & $0.018\pm 0.019$ & $0$ & $0.002\pm 0.002$ & $0.007\pm 0.008$  \\
VV           & $0.230\pm 0.091$ & $0.195\pm 0.078$ & $0.177\pm 0.071$ & $0.159\pm 0.065$ & $0.124\pm 0.051$ & $0.115\pm 0.048$  \\\hline
\Bexp        & $1.614\pm 0.301$ & $1.354\pm 0.240$ & $1.887\pm 0.367$ & $1.339\pm 0.189$ & $2.142\pm 0.351$ & $2.136\pm 0.302$  \\\hline
$S$          & $0.209\pm 0.054$ & $0.183\pm 0.048$ & $0.161\pm 0.042$ & $0.130\pm 0.034$ & $0.121\pm 0.031$ & $0.102\pm 0.027$  \\\hline
\Nobs        & $     1$         &	   $2$     &	  $2$	      & $2$ 	         & $3$		    & $     3$       		  \\
\hline\hline
\end{tabular}
}
\end{center}
\end{table}

\begin{table}[htbp]
\caption{Predicted backgrounds including the statistical uncertainty and the
systematic uncertainty from the control region and b-tag scale factors, signal 
yields with total uncertainty, and the observed number of events for each mass 
point in the \ZnnH\ BDT analysis.}
\label{tab:ZnnHBDTYields}
\begin{center}
\scalebox{0.8}{
\begin{tabular}{ccccccc} \hline\hline
Process       & $110\GeV$        & $115\GeV$        & $120\GeV$        & $125\GeV$        & $130\GeV$        & $135\GeV$        \\\hline
%\Wudscg       & $0$              & $0$              & $0$              & $0.001\pm 0.001$ & $0$              & $0$ \\
\Wbb + \ttbar & $0.656\pm 0.197$ & $0.656\pm 0.197$ & $0.525\pm 0.158$ & $0.787\pm 0.236$ & $0.263\pm 0.079$ & $0.394\pm 0.118$ \\
\Zudscg       & $0.581\pm 0.126$ & $0.113\pm 0.025$ & $0.174\pm 0.038$ & $0.222\pm 0.048$ & $0.281\pm 0.061$ & $0.341\pm 0.074$ \\
\Zbb          & $1.256\pm 0.384$ & $1.108\pm 0.339$ & $1.182\pm 0.362$ & $0.936\pm 0.286$ & $1.207\pm 0.369$ & $1.034\pm 0.316$ \\
ST            & $0.452\pm 0.171$ & $0.453\pm 0.172$ & $0.432\pm 0.164$ & $0.411\pm 0.156$ & $0.543\pm 0.206$ & $0.853\pm 0.323$ \\
VV            & $0.843\pm 0.319$ & $0.571\pm 0.216$ & $0.252\pm 0.095$ & $0.291\pm 0.110$ & $0.063\pm 0.024$ & $0.351\pm 0.133$ \\\hline
\Bexp         & $3.992\pm 0.730$ & $2.901\pm 0.572$ & $2.565\pm 0.500$ & $2.648\pm 0.510$ & $2.357\pm 0.475$ & $2.973\pm 0.596$ \\\hline
$S$           & $0.642\pm 0.167$ & $0.548\pm 0.142$ & $0.352\pm 0.092$ & $0.317\pm 0.082$ & $0.259\pm 0.067$ & $0.216\pm 0.056$ \\\hline
\Nobs         & $2$              & $1$   	    & $1$	       & $5$   	          & $2$   	     & $3$              \\
\hline\hline
\end{tabular}
}
\end{center}
\end{table}



\begin{figure}[htbp]
  \begin{center}
%     \includegraphics[width=0.48\textwidth]{figures/WmnHmassCCLog.pdf}
%    \includegraphics[width=0.48\textwidth]{figures/WenHmassCCLog.pdf}
%    \includegraphics[width=0.48\textwidth]{figures/ZmmHmassCCLog.pdf}
%    \includegraphics[width=0.48\textwidth]{figures/ZeeHmassCCLog.png}
%    \includegraphics[width=0.48\textwidth]{figures/ZnnHmassCCLog.pdf}
    \includegraphics[width=0.49\textwidth]{figures/CCWm_Aug18.pdf}
    \includegraphics[width=0.49\textwidth]{figures/CCWe_Aug18.pdf}
    \includegraphics[width=0.49\textwidth]{figures/CCZmm_Aug18.pdf}
    \includegraphics[width=0.49\textwidth]{figures/CCZee_Aug18.pdf}
    \includegraphics[width=0.49\textwidth]{figures/CCZnn_Aug18.pdf}
    \caption{Distributions of dijet invariant mass after all \Mbb\
    selection criteria have been applied in (clockwise from top left to
    bottom right: \WmnH, \WenH, \ZmmH, \ZeeH, \ZnnH.}
    \label{fig:MassCC}
  \end{center}
\end{figure}


\begin{figure}[htbp]
  \begin{center}
%    \includegraphics[width=0.49\textwidth]{figures/WmnHBDTDataLog.pdf}
%   \includegraphics[width=0.49\textwidth]{figures/WenHBDTDataLog.pdf}
%    \includegraphics[width=0.49\textwidth]{figures/ZmmHBDTDataLog.pdf}
%    \includegraphics[width=0.49\textwidth]{figures/ZeeHBDTDataLog}
%    \includegraphics[width=0.49\textwidth]{figures/ZnnHBDTDataLog.pdf}
    \includegraphics[width=0.49\textwidth]{figures/BDTWm_Aug18.pdf}
    \includegraphics[width=0.49\textwidth]{figures/BDTWe_Aug18.pdf}
    \includegraphics[width=0.49\textwidth]{figures/BDTZmm_Aug18.pdf}
    \includegraphics[width=0.49\textwidth]{figures/BDTZee_Aug18.pdf}
    \includegraphics[width=0.49\textwidth]{figures/BDTZnn_Aug18.pdf}
    \caption{Distributions of BDT output for  data (points with
      errors) and all backgrounds: 
\WmnH\ (top left), \WenH\ (top right), \ZmmH\ (middle left), \ZeeH\ (middle right)
      and \ZnnH\ )bottom.
}
    \label{fig:BDTdata}
  \end{center}
\end{figure}



\clearpage


\subsection{Upper limits}

Preliminary  $95\%$ C.L. upper limits on the Higgs production
cross section in the VH mode with \HBB\ were obtained from both
the BDT and \Mjj\ analyses for a dataset corresponding to an integrated
luminosity of  $ 1.1$~fb$^{-1}$.  The limits were calculated using the 
LandS code~\cite{LandS}.  The results were also checked with the standard 
RooStats configuration~\cite{RooStats}, and found to be consistent.
For the expected and observed limits, and the 1- and 2-$\sigma$ bands,
the CLs method currently recommended by the LHC Higgs Combination Group 
was employed~\cite{HIG-11-011}. Signal and background uncertainties, as 
described in the previous sections, were included as nuisance parameters 
in the calculation, with appropriate correlations taken into account.

The results of the five \BDT\ analyses are combined to produce limits on 
Higgs production in the \bbbar\ channel for the assumed masses:
$110-135$~GeV.  The identical procedure was applied to the results of the 
\Mbb\ analysis. Table~\ref{tab:Limits}
summarizes the resulting, expected and observed, upper $95\%$
C.L. cross section limits,
with respect to the standard model cross section, for each of the mass 
points for the \BDT\ and \Mbb\ analyses. The results are displayed separately
in Fig.~\ref{fig:Limits}.  The primary result is the one from the \BDT\ analysis.

%The expected Bayesian limits are compared to the CLs 
%results in Fig.~\ref{fig:BayesLimits}.

\begin{figure}[tbp]
  \begin{center}
%    \includegraphics[width=0.49\textwidth]{figures/BDTlimitCLs.pdf}
%    \includegraphics[width=0.49\textwidth]{figures/CClimitCLs.pdf}
    \includegraphics[width=0.49\textwidth]{figures/BDTLimits_Lands_Aug19.pdf}
    \includegraphics[width=0.49\textwidth]{figures/CCLimits_Lands_Aug19.pdf}
    \caption{Expected and observed $95\%$ C.L. combined upper limits on the ratio of
    VHbb production for the BDT (left) and \Mjj\ (right) analyses.  The median expected
    limit and the 1- and 2-$\sigma$ bands are obtained with the LHC CLs method as
    implemented in LandS, as are the observed limits at each mass point.}
    \label{fig:Limits}
  \end{center}
\end{figure}



\begin{table}[tbp]
\caption{Expected and observed $95\%$ CL upper limits on the 
production of a SM Higgs boson in association with W and Z bosons
and decaying to b quarks relative to the expected cross section.
Limits are listed separately for the \BDT\ and \Mbb\ analyses.}
\label{tab:Limits}
\begin{center}
\begin{tabular}{ccccc} \hline\hline
\MH(\GeV) & \BDT\ Expected & \BDT\ Observed & \Mjj\ Expected & \Mjj\ Observed \\  \hline
 110      & $5.8$        & $8.0$        & $6.4$          & $8.2$          \\
 115      & $5.7$        & $8.3$        & $6.0$          & $11.3$         \\
 120      & $7.7$        & $9.5$        & $8.1$          & $11.4$         \\
 125      & $9.6$        & $15.3$       & $8.6$          & $11.6$         \\
 130      & $11.0$       & $16.3$       & $12.1$         & $14.0$         \\
 135      & $14.4$       & $22.5$       & $15.0$         & $19.9$         \\
\hline\hline
\end{tabular}
\end{center}
\end{table}


==> HIG-11-012/trunk/HIG-11-012-simulation.tex <==

Simulated samples of signal and backgrounds were produced using
various event generators, with the CMS detector response modeled in
extensive detail with {\tt GEANT4}~\cite{GEANT4}. The Higgs signal samples were
produced using {\tt POWHEG}~\cite{POWHEG} interfaced with the {\tt HERWIG}~\cite{HERWIG} parton shower
generator. The diboson samples come from {\tt Pythia6}~\cite{Pythia} and
{\tt MadGraph}~\cite{MadGraph} is used for W+jets and Z+jets.
For $t\bar t$ production the simulated samples were produced using
{\tt MadGraph}. The single-top samples were produced with {\tt POWHEG} and the QCD
samples with {\tt Pythia}. All samples were generated with a roughly flat pileup (PU)
distribution up to 10 interactions per proton bunch crossings. The
PU interactions are overlapping minimum-bias events added at random within
the proton-proton interaction region.
During the period in which the data for this analysis was recorded the
LHC instantaneous luminosity reached up to $\sim 1.4\cdot{\rm e}^{33}{\rm
cm}^{-2}{\rm s}^{-1}$ and 
the average number of interactions per bunch crossing was
about six. The simulated samples were reweighted to represent the PU
distribution measured in the data.




==> HIG-11-012/trunk/HIG-11-012-syst.tex <==
The primary physics result described in this note is an upper limit
on the production of a standard model Higgs boson produced in 
association with a vector boson and decaying to a \bbbar\ pair.

The following systematic uncertainties on the expected signal and background
yields affect the upper limit. The values listed are an approximation of
what is actually used in the limit calculation.

\begin{itemize}
\item {\bf Luminosity}: The CMS luminosity uncertainty for this
  dataset was estimated to be $4.5\%$.

 \item {\bf Lepton Efficiency}: muon and electron trigger, 
       reconstruction, and identification efficiencies are 
       determined in data using the standard tag-and-probe
       technique (TnP) with Z bosons.  The systematic uncertainty
       is evaluated from the statistical uncertainties in the
       bin-by-bin efficiencies and scale factors as applied to 
       signal Monte Carlo samples.  The total uncertainty is
       $\sim 2\%$ per lepton.

 \item {\bf MET+jets Trigger}: the parameters describing the
       trigger efficiency curve have been
       varied within their statistical uncertainties.  An
       uncertainty of $+1.5,-3.2\%$ was estimated \ZnnH.

 \item {\bf Unclustered MET}: An uncertainty of $3\%$ is assigned to
   the yields due to energy fluctuations not associated to jets.

 \item {\bf Jet Energy Scale (JES)}: the jet energy scale was
       varied within one standard deviation based on $\pt$ and 
       $\eta$, and the efficiency of the analysis selection was
       recomputed to assess the systematic variation.  An uncertainty of $1\%$
       was obtained.

 \item {\bf Jet Energy Resolution (JER)}: the effect of uncertainty
       on the jet energy resolution was evaluated by
       scaling the measured resolution on a jet-by-jet basis.  An 
       uncertainty of $\sim 10\%$ was measured for all processes.

 \item {\bf B-jet Tagging}: b-tagging data to simulation scale factors
   are applied  consistently to jets in signal and background
       events. A systematic uncertainty of $10\%$,
   per b-tag, is assigned to all channels. 

 \item {\bf Signal cross section}: the total cross section has 
       been calculated to next-to-next-to-leading order accuracy, 
       and the total uncertainty is $4\%$~\cite{LHCHiggsWG,VHatNNLO}, including
       the effect of scale and PDF variations.

 \item {\bf Theoretical H \pt\ Spectrum}: this analysis is performed
       in the boosted regime, and thus, potential differences in
       the \pt\ spectrum of the V and H between data and Monte
       Carlo generators could introduce systematic effects in the
       signal acceptance and efficiency estimates.  Recently, two 
       calculations have become available that estimate the NLO
       electroweak~\cite{HAWK1,HAWK2,HAWK3} and NNLO QCD~\cite{Grazzini} 
       corrections to VH production in the boosted regime.  The estimated
       effect from electroweak corrections for a boost of $\sim 150\GeV$
       are $5\%$ for ZH and $10\%$ for WH.  For the QCD correction, the
       relevant comparison is NNLO vs. NLO, where an uncertainty of 
       $10\%$ for both ZH and WH is estimated. 

 \item {\bf Background Estimate}: a mix of data-driven methods,
       simulation, and theory uncertainties contribute to the total
       uncertainty on the background estimates, which are listed in
       Tables~\ref{tab:WmnHCCyields}--\ref{tab:ZnnHBDTYields}.  
       Correlated (luminosity, b-tagging, JEC/JER,
       and TnP efficiencies) and uncorrelated uncertainties (statistical,
       control region, and cross section) are combined separately.
       An uncertainty of $30\%$ is assumed for single top (approximately
       the uncertainty on the measured cross section) and diboson (assumed
       to have the same uncertainty as the signal).  The other backgrounds
       are taken directly from data, with the associated uncertainties
       from the control regions.
 \item {\bf Monte Carlo Statistics}: the finite size of the signal
       Monte Carlo signal samples contributes $4\%$ across all channels,
       while the background statistical uncertainty can be large depending
       on the channel and the background source.

\end{itemize}

The total uncertainty on the signal prediction is taken to be $26\%$ and 
$28\%$ for ZH and WH production, respectively.  Background uncertainties 
range from $12\%$ to $20\%$ depending on mode and mass point.


==> HIG-11-012/trunk/HIG-11-012-trigger.tex <==
Several triggers were used to collect events consistent with
the signal hypothesis in all five channels.
 
For the WH channels the trigger paths require single-lepton
triggers with tight lepton identification, calorimeter and tracker
isolation requirements applied to maintain an acceptable trigger
rate. For the \WmnH\ channel the \PT\ threshold for the muon trigger was 17\GeV. 
This trigger was used for the complete dataset and was 70-95\%
efficient, depending on rapidity and
\pt\ . Its effective efficiency for muons from signal,
reconstructed offline with \PT\ $>20$\GeV, was $\sim 90\%$. For the
\WenH\ channel the trigger for the first 200~pb$^{-1}$ of data
required a single electron with \ET\ $>27$\GeV. The effective
efficiency was $\sim 95\%$ for electrons reconstructed offline with
\ET\ $>30$\GeV. For the next $\sim 300$~pb$^{-1}$ the
single electron trigger threshold was reduced to 17\GeV by adding the
requirement of two jets and pfMHT -which is the resulting missing
transverse energy (\MET\ ) when adding up the transverse energy of all jets
reconstructed with a particle flow
algorithm~\cite{CMS-PAS-JME-10-003}. The jets \ET thresholds were 30
and 25\GeV for the leading and sub-leading jet, respectively. The
pfMHT threshold was 15\GeV. For the last $\sim 600$~pb$^{-1}$ the
electron and pfMHT thresholds were raised to 22 and 30\GeV, respectively.
The effective efficiency for these triggers for signal events that
pass the final offline selection criteria in Section~\ref{sec:event-sel} was $\sim$97\%.

For the \ZmmH\ channel the same single muon trigger, described above,
was used; while for the \ZeeH\ channel, a di-electron trigger with lower \ET
thresholds $17/8$ \GeV and very tight isolation requirements was used.
Both of these triggers were $\sim 99\%$ efficient for the  $20/20$
\GeV \PT\ (\ET\ ) offline threshold
combination used on both muons (electrons).  

For the \ZnnH\ channel, combinations of three triggers were used. The first one required
pfMHT$>150\GeV$ and was used for the complete dataset. The second and
third one allow a 
lower \MET\ threshold of 80 GeV (reconstructed from all energy
deposits in the calorimeter). For the second one the presence of a central
jet  ($|\eta|<2.4$) above a \ET\ threshold of 80\GeV was required, and for the
third trigger the requirement was that there be 
two central jets with \ET
$>20 \GeV$. For the first $\sim 200$~pb$^{-1}$ of data events were
required to pass the {\tt OR} of
the first two triggers and for the last $\sim 900$~pb$^{-1}$ the
requirement was that they pass the {\tt OR} of the first and third
trigger. The effective trigger efficiency was 50\% for an
offline pfMET of 120\GeV and $\sim 98\%$ above
the 160\GeV threshold used for the offline event selection.
The relatively high \MET\ thresholds were needed to keep the trigger rate under control.


==> HIG-11-012/trunk/HIG-11-012.tex <==
% Customizable fields and text areas start with % >> below.
% Lines starting with the comment character (%) are normally removed before release outside the collaboration, but not those comments ending lines

%JK NOTES =========
%================
% check consistency of tense => PAST for preparations, PRESENT for action



% Useful aliases
\newcommand\T{\rule{0pt}{2.3ex}}
\newcommand\B{\rule[-1.0ex]{0pt}{0pt}}
% Jaco's &&&
%
\def\Mbb   {\ensuremath{M(\mathrm{jj})}}
%\def\Mbb   {\ensuremath{\mathrm{M_{\bbbar}}}}
\def\BDT {{\tt BDT}}
\def\Zj  {\ensuremath{\mathrm{Z + jets}}}
\def\Wj  {\ensuremath{\mathrm{W + jets}}}
\def\Vj  {\ensuremath{\mathrm{V + jets}}}
\def\VtoBB {\ensuremath{\mathrm{V}\to\bbbar}}
\def\mH{\ensuremath{\mathrm{m}_H}}
\def\HT{\ensuremath{\mathrm{H}_T}}



%
%
%==================
\def\ZnnH  {\ensuremath{\mathrm{Z}(\cPgn\cPgn)\mathrm{H}}}
\def\ZllH  {\ensuremath{\mathrm{Z}(\ell\ell)\mathrm{H}}}
\def\ZmmH  {\ensuremath{\mathrm{Z}(\Pgm\Pgm)\mathrm{H}}}
\def\ZeeH  {\ensuremath{\mathrm{Z}(\Pe\Pe)\mathrm{H}}}
\def\WlnH  {\ensuremath{\mathrm{W}(\ell\cPgn)\mathrm{H}}}
\def\WmnH  {\ensuremath{\mathrm{W}(\Pgm\cPgn)\mathrm{H}}}
\def\WenH  {\ensuremath{\mathrm{W}(\Pe\cPgn)\mathrm{H}}}
\def\WtoLN {\ensuremath{\mathrm{W}\to\ell\cPgn}}
\def\WtoEN {\ensuremath{\mathrm{W}\to\Pe\cPgn}}
\def\WtoMN {\ensuremath{\mathrm{W}\to\Pgm\cPgn}}
\def\ZtoBB {\ensuremath{\mathrm{Z}\to\bbbar}}
\def\ZtoNN {\ensuremath{\mathrm{Z}\to\cPgn\bar{\cPgn}}}
\def\ZtoLL {\ensuremath{\mathrm{Z}\to\ell\ell}}
\def\ZtoMM {\ensuremath{\mathrm{Z}\to\MM}}
\def\ZtoEE {\ensuremath{\mathrm{Z}\to\EE}}
\def\ZmmJ  {\ensuremath{\mathrm{Z}(\Pgm\Pgm)\mathrm{+jets}}}
\def\ZnnJ  {\ensuremath{\mathrm{Z}(\cPgn\bar{\cPgn})\mathrm{+jets}}}
\def\WJ  {\ensuremath{\mathrm{W + jets}}}
\def\HBB   {\ensuremath{\mathrm{H}\to\bbbar}}
\def\HTT   {\ensuremath{\mathrm{H}\to\TT}}
\def\mtW   {\ensuremath{M_{\mathrm{T}}}}
\def\ptl   {\ensuremath{p_{\mathrm{T}}^{\ell}}}
\def\MyZ   {\ensuremath{\mathrm{Z}}}
\def\MyW   {\ensuremath{\mathrm{W}}}
\def\MyH   {\ensuremath{\mathrm{H}}}
\def\Vudscg   {\ensuremath{\mathrm{V+udscg}}}
\def\Wudscg   {\ensuremath{\mathrm{W+udscg}}}
\def\Wenudscg   {\ensuremath{\mathrm{W}(\Pe\cPgn)+\mathrm{udscg}}}
\def\Wmnudscg   {\ensuremath{\mathrm{W}(\Pgm\cPgn)+\mathrm{udscg}}}
\def\Wenbb   {\ensuremath{\mathrm{W}(\Pe\cPgn)+\bbbar}}
\def\Wmnbb   {\ensuremath{\mathrm{W}(\Pgm\cPgn)+\bbbar}}
\def\Zeebb   {\ensuremath{\mathrm{Z}(\Pe\Pe)+\bbbar}}
\def\Zmmbb   {\ensuremath{\mathrm{Z}(\Pgm\Pgm)+\bbbar}}
\def\Zudscg   {\ensuremath{\mathrm{Z+udscg}}}
\def\Zeeudscg   {\ensuremath{\mathrm{Z}(\Pe\Pe)+\mathrm{udscg}}}
\def\Zmmudscg   {\ensuremath{\mathrm{Z}(\Pgm\Pgm)+\mathrm{udscg}}}
\def\Zenbb   {\ensuremath{\mathrm{Z}(\Pe\cPgn)+\bbbar}}
\def\Zmnbb   {\ensuremath{\mathrm{Z}(\Pgm\cPgn)+\bbbar}}
\def\Wbb   {\ensuremath{\mathrm{W\bbbar}}}
\def\Zbb   {\ensuremath{\mathrm{Z\bbbar}}}
\def\Vbb   {\ensuremath{\mathrm{V\bbbar}}}
\def\Zll   {\ensuremath{Z(\ell\ell)}}
\def\Mjj   {\ensuremath{M(\mathrm{jj})}}
\def\ptjj   {\ensuremath{{\pt}(\mathrm{jj})}}
\def\MZ {\ensuremath{M_{\mathrm{Z}}}}
\def\dRJJ {\ensuremath{\Delta R(\mathrm{J1,J2})}}
\def\dEtaJJ {\ensuremath{\Delta \eta(\mathrm{J1,J2})}}
\def\dphiVH {\ensuremath{\Delta\phi(\mathrm{V,H})}}
\def\dphiWH {\ensuremath{\Delta\phi(\mathrm{W,H})}}
\def\dphiZH {\ensuremath{\Delta\phi(\mathrm{Z,H})}}
\def\dphiMJ {\ensuremath{\Delta\phi(\mathrm{pfMET,J})}}
\def\cosTH {\ensuremath{\cos{\theta^*}}}
\def\dThPull {\ensuremath{\Delta\theta_{\mathrm{pull}}}}
\def\ptV {\ensuremath{p_{\mathrm{T}}(\mathrm{V})}}
\def\ptH {\ensuremath{p_{\mathrm{T}}(\mathrm{H})}}
\def\ptZ {\ensuremath{p_{\mathrm{T}}(\mathrm{Z})}}
\def\ptW {\ensuremath{p_{\mathrm{T}}(\mathrm{W})}}
\def\Naj {\ensuremath{N_{\mathrm{aj}}}}
\def\Nal {\ensuremath{N_{\mathrm{al}}}}
\def\etaTF {\ensuremath{\left | \eta \right | < 2.5}}
\def\Bexp {\ensuremath{B_{\mathrm{exp}}}}
\def\Bobs {\ensuremath{B_{\mathrm{obs}}}}
\def\Nobs {\ensuremath{N_{\mathrm{obs}}}}


% svn info. These are modified by svn at checkout time.
% The last version of these macros found before the maketitle will be the one on the front page,
% so only the main file is tracked.
% Do not edit by hand!
\RCS$Revision: 61381 $
\RCS$HeadURL: svn+ssh://svn.cern.ch/reps/tdr2/notes/HIG-11-012/trunk/HIG-11-012.tex $
\RCS$Id: HIG-11-012.tex 61381 2011-06-15 19:42:54Z alverson $
%%%%%%%%%%%%% ptdr definitions %%%%%%%%%%%%%%%%%%%%%
%\input{ptdr-definitions} %These have been replaced by the equivalent style file
%%%%%%%%%%%%%%%  Title page %%%%%%%%%%%%%%%%%%%%%%%%
\cmsNoteHeader{HIG-11-012} % This is over-written in the CMS environment: useful as preprint no. for export versions
% >> Title: please make sure that the non-TeX equivalent is in PDFTitle below
\title{Search for the Standard Model Higgs Boson Decaying to Bottom
  Quarks and Produced in Association with a W or a Z Boson}

% >> Authors
%Author is always "The CMS Collaboration" for PAS and papers, so author, etc, below will be ignored in those cases
%For multiple affiliations, create an address entry for the combination
\address[neu]{University of Florida}
\address[fnal]{Fermilab}
\address[cern]{CERN}
\author[cern]{The CMS Collaboration}

% >> Date
% The date is in yyyy/mm/dd format. Today has been
% redefined to match, but if the date needs to be fixed, please write it in this fashion.
% For papers and PAS, \today is taken as the date the head file (this one) was last modified according to svn: see the RCS Id string above.
% For the final version it is best to "touch" the head file to make sure it has the latest date.
\date{\today}

% >> Abstract
% Abstract processing:
% 1. **DO NOT use \include or \input** to include the abstract: our abstract extractor will not search through other files than this one.
% 2. **DO NOT use %**                  to comment out sections of the abstract: the extractor will still grab those lines (and they won't be comments any longer!).
% 3. **DO NOT use tex macros**         in the abstract: External TeX parsers used on the abstract don't understand them.
\abstract{
   A search for the standard model Higgs boson is performed in a data
   sample corresponding to an integrated luminosity of $1.1$~fb$^{-1}$, recorded by the CMS detector
   in proton-proton collisions at the LHC with a 7~TeV center-of-mass energy.
   The following modes are studied: $W(\mu\nu)H,~ W(e\nu)H,~
   Z(\mu\mu)H,~ Z(ee)H$ and $Z(\nu\nu)H$, with the Higgs decaying to
   $b\bar{b}$ pairs. 95\% C.L. upper limits on the
  VH production cross section are derived for a Higgs mass between
   110 and 135 GeV. The expected (observed) upper limit at 115~GeV is
  found to be 5.7 (8.3) times
   the standard model expectation. 
}

% >> PDF Metadata
% Do not comment out the following hypersetup lines (metadata). They will disappear in NODRAFT mode and are needed by CDS.
% Also: make sure that the values of the metadata items are sensible. For APS submissions, they are automatically converted to APS keywords.
\hypersetup{%
pdfauthor={Jacobo Konigsberg},%
pdftitle={Search for the Standard Model Higgs Boson Decaying to Bottom Quarks and Produced in Association with a W or a Z Boson},%
pdfsubject={CMS},%
pdfkeywords={CMS, physics, Higgs}}

\maketitle %maketitle comes after all the front information has been supplied

% >> Text
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Begin text %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% **DO NOT REMOVE THE BIBLIOGRAPHY** which is located before the appendix.
%% You can take the text between here and the bibiliography as an example which you should replace with the actual text of your document.
%% If you include other TeX files, be sure to use "\input{filename}" rather than "\input filename".
%% The latter works for you, but our parser looks for the braces and will break when uploading the document.
%%%%%%%%%%%%%%%



\section{Introduction}\label{sec:intro}
\input{HIG-11-012-intro.tex}


\section{The CMS Detector and Simulated Samples}\label{sec:detector}
\input{HIG-11-012-detector.tex}
\input{HIG-11-012-simulation.tex}


\section{Trigger and Event Reconstruction}\label{sec:trigger_event}
\input{HIG-11-012-trigger.tex}
\input{HIG-11-012-event-rec.tex}


\section{Event Selection}\label{sec:event-sel}
\input{HIG-11-012-event-sel.tex}


\section{Background Control Regions}\label{sec:bck-ctrl}
\input{HIG-11-012-bck-ctrl.tex}

\section{Systematic Uncertainties}\label{sec:sys}
\input{HIG-11-012-syst.tex}

\section{Results}\label{sec:results}
\input{HIG-11-012-results.tex}

\section{Conclusions}\label{sec:conclusions}
\input{HIG-11-012-conclusions.tex}




%===================================
%===================================


%% **DO NOT REMOVE BIBLIOGRAPHY**
\bibliography{auto_generated}   % will be created by the tdr script.

%% examples of appendices. **DO NOT PUT \end{document} at the end
%\clearpage
%\appendix
%\section{A-1}}

%%% DO NOT ADD \end{document}!


